Millimeter light curves of Sagittarius A* observed during the 2017 Event Horizon Telescope campaign

The Event Horizon Telescope (EHT) observed the compact radio source, Sagittarius A* (Sgr A*), in the Galactic Center on 2017 April 5-11 in the 1.3 millimeter wavelength band. At the same time, interferometric array data from the Atacama Large Millimeter/submillimeter Array and the Submillimeter Array were collected, providing Sgr A* light curves simultaneous with the EHT observations. These data sets, complementing the EHT very-long-baseline interferometry, are characterized by a cadence and signal-to-noise ratio previously unattainable for Sgr A* at millimeter wavelengths, and they allow for the investigation of source variability on timescales as short as a minute. While most of the light curves correspond to a low variability state of Sgr A*, the April 11 observations follow an X-ray flare, and exhibit strongly enhanced variability. All of the light curves are consistent with a red noise process, with a power spectral density (PSD) slope measured to be between -2 and -3 on timescales between 1 min and several hours. Our results indicate a steepening of the PSD slope for timescales shorter than 0.3 h. The spectral energy distribution is flat at 220 GHz and there are no time-lags between the 213 and 229 GHz frequency bands, suggesting low optical depth for the event horizon scale source. We characterize Sgr A*'s variability, highlighting the different behavior observed just after the X-ray flare, and use Gaussian process modeling to extract a decorrelation timescale and a PSD slope. We also investigate the systematic calibration uncertainties by analyzing data from independent data reduction pipelines.

==> old_version_table_all_data.tex <==
\begin{table*}[th!]
     \caption{Archival \sgra light curves \rev{at frequency $\sim$\,230\,GHz} from the literature.
     }
    \begin{center}
    \tabcolsep=0.2cm
    \begin{tabularx}{0.92\linewidth}{lclcccccc}
    \hline
    \hline
     Reference & Array & Date &  Duration (h) & Samples & Flux (Jy) & $\sigma/\mu$ & max-min (Jy) \\
     \hline
     \citet{Marrone2006} & SMA & 2005 June 4 & 3.3 & 15 & $3.99\pm 0.44$ & 0.109 & 1.31 \\
               &  & 2005 June 9 & 5.9 & 32 & $3.41\pm 0.24$ & 0.071 & 1.01 \\
               & & 2005 June 16 & 6.5 & 45 & $3.85\pm0.34$ & 0.087 & 1.07 \\
               & & 2005 July 20 & 5.3 & 32 & $3.78\pm0.27$ & 0.070 & 0.86 \\
               & & 2005 July 22 & 5.4 & 33 & $3.36\pm0.24$ & 0.071 & 0.87 \\
               & & 2005 July 30 & 6.8 & 33 & $4.12\pm0.42$ & 0.103 & 1.95 \\
     
    \hline
    %\multirow{3}{4em}{ALMA} 
    \citet{Marrone2008} & SMA  & 2006 July 17 &  6.3 & 45 & $3.04\pm0.25$ &0.081 & 0.97 \\
    \hline
     \citet{Yusef2009} & SMA  & 2007 April 1 &  6.3 & 13 & $3.35\pm0.25$ &0.074 & 0.73  \\
       &   & 2007 April 3 &  5.3 & 35 & $3.32\pm0.35$ &0.104 &1.14 \\
        &   & 2007 April 4 &  6.4 & 41 & $2.82\pm0.11$ &0.038 &0.45 \\
         &   & 2007 April 5 &  6.5 & 32 & $2.84\pm0.28$ &0.097 &0.91 \\
    \hline
    
    \citet{Dexter2014} & CARMA$^a$  & 2009 April 5 &  3.9 & 46 & $3.23\pm0.26$ &0.081 & 0.98\\
      &   & 2009 April 6 &  3.8 & 42 & $3.33\pm0.29$ &0.088& 1.13 \\
       &   & 2011 March 29 &  4.2 & 36 & $3.03\pm0.57$ &0.187 &2.14 \\
       &   & 2011 March 31 &  3.2 & 25 & $2.89\pm0.29$ &0.102 &0.84 \\
        &   & 2011 April 1 &  4.2 & 32 & $2.99\pm0.17$ &0.059 &0.73 \\
         &   & 2011 April 4 &  3.7 & 39 & $3.49\pm0.37$ &0.107& 1.72 \\
        &   & 2012 May 4 &  4.6 & 50 & $3.58\pm0.27$ &0.077 &1.24 \\
        &   & 2012 May 10 &  4.3 & 48 & $3.89\pm0.38$ &0.097 &1.71 \\
     \cline{2-8}
     & SMA  & 2012 May 16 &  7.6 & 82 & $4.13\pm0.28$ &0.067 & 1.35\\
      &   & 2012 May 17 &  7.5 & 76 & $3.94\pm0.31$ &0.078& 2.02 \\
       &   & 2012 May 18 &  7.0 & 60 & $3.91\pm0.43$ &0.110 &2.23 \\
       &   & 2012 May 19 &  6.7 & 68 & $4.21\pm0.20$ &0.047 &0.98 \\
        &   & 2012 July 20 &  3.8 & 25 & $2.50\pm0.20$ &0.081 &0.69 \\
         &   & 2012 July 21 &  2.3 & 24 & $4.13\pm0.12$ &0.030& 0.51 \\
        &   & 2012 July 22 &  4.0 & 32 & $3.29\pm0.17$ &0.052 &0.73 \\
        &   & 2012 July 23 &  2.5 & 22 & $2.90\pm0.34$ &0.117 &0.99 \\
        \hline

     \citet{fazio:2018} & SMA  & 2015 May 14 &  5.7 & 439 & $5.25\pm0.36$ &0.069 & 1.56 \\
        \hline
        
     \citet{Bower2018} & ALMA  & 2016 March 3 &  3.0 & 40 & $3.92\pm0.16$ &0.040 & 0.72 \\
      & %226.0\,GHz  
      & 2016 May 3 &  3.0 & 45 & $3.21\pm0.17$ &0.054 &0.62 \\
      &   & 2016 August 13 &  6.4 & 26 & $2.66\pm0.28$ &0.103 & 0.82 \\
        \hline
        
    \citet{Witzel2021} & SMA  & 2016 July 13 &  6.5 & 798 & $3.71\pm0.22$ &0.059 & 0.82 \\
      & & 2017 July 15 &  7.7 & 1671 & $2.75\pm0.27$ &0.098 &1.45 \\
      &   & 2017 July 25 &  6.0 & 1280 & $2.37\pm0.15$ &0.064 & 0.91 \\
      
      \cline{2-8}
      
      & ALMA  & 2016 July 12 &  4.7 & 78 & $4.00\pm0.09$ &0.023 & 0.34 \\
      & %226.0\,GHz  
      & 2016 July 18 &  6.5 & 88 & $3.20\pm0.34$ &0.106 &1.13 \\
   
      
      
        \hline
        
\citet{Iwata2020} & ALMA  & 2017 October 5 &  1.2 & 44 & $2.85\pm0.07$ &0.023 & 0.21 \\
 &  %234.0\,GHz 
 & 2017 October 7 &  1.2 & 45 & $3.20\pm0.08$ &0.025 &0.23\\
  &  & 2017 October 8 &  1.2 & 44 & $3.11\pm0.08$ &0.027 & 0.30 \\
    &  & 2017 October 10 &  1.2 & 45 & $3.27\pm0.05$ &0.017 & 0.18 \\
     &  & 2017 October 11a &  1.2 & 45 & $3.25\pm0.06$ &0.020 &  0.23 \\
     &  & 2017 October 11b &  1.2 & 44 & $2.96\pm0.05$ &0.016 & 0.16 \\
     &  & 2017 October 14 &  1.2 & 44 & $3.00\pm0.03$ &0.009 & 0.11 \\
     &  & 2017 October 17 &  1.2 & 45 & $2.63\pm0.12$ &0.047 & 0.36 \\
     &  & 2017 October 18 &  1.2 & 44 & $2.08\pm0.08$ &0.040 & 0.23\\
     &  & 2017 October 19 &  1.2 & 45 & $3.04\pm0.05$ &0.018 & 0.18 \\
     
  \hline
  
\citet{Murchikova2021} & ALMA  & 2019 June 12 &  1.2 & 1252 & $4.62\pm0.06$ &0.013 & 0.27 \\
 &  %234.0\,GHz 
 & 2019 June 13 &  1.2 & 1286 & $3.14\pm0.05$ &0.015 &0.22\\
  &  & 2019 June 14 &  1.2 & 1267 & $3.33\pm0.13$ &0.039 & 0.49 \\
    &  & 2019 June 20 &  1.2 & 1305 & $3.59\pm0.07$ &0.021 & 0.25 \\
&  & 2019 June 21 &  4.6 & 3913 & $3.85\pm0.19$ &0.050 & 0.68 \\

    \hline 
    \hline
    \end{tabularx}
    %\label{tab:detections_other_papers}
    \end{center}
    $^a$Combined Array for Research in Millimeter-wave Astronomy, Cedar Flat, California, USA
\end{table*}

